Deal With It: On Better Schedules for Listwise Reranking

Listwise LLM rerankers cannot reliably rank hundreds of documents in a single call, and rely on schedules to orchestrate their calls. Parallel schedules split candidates into groups and advance a fixed quota from each. When a group holds more of the top passages than its quota, some are cut, and expensive repair calls become required. We show that the way candidates are split matters where such a quota can bind, and that, in expected cuts, the best split there deals them round-robin by retriever rank, like cards. Although not conceptually new, dealing has remained unanalyzed. We prove that, under a simple retriever model, no split with equal quotas cuts fewer of the true top ten on average, and that contiguous chunks cut more as the retriever improves. DealRank, the simplest schedule our analysis allows, is on average within 0.1 nDCG@10 points of the best schedules over six LLMs, in two rounds. It is consistently 1.1 to 1.4 times faster than BlitzRank with concurrent first calls up to a thousand candidates. There, it needs three rounds and is eleven times faster than the sliding window. In existing schedules such as BlitzRank, dealing reduces repair calls from 59% of queries to 14%, improving latency with no significant change in quality. Random partitioning appears equivalent at a quota of four, as predicted, but ties results to the seed and trails by 1.3 nDCG@10 points at a quota of one over a dense retriever.

==> figures/fig2.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig2_split_v2.pdf}
  \caption{Expected (lines) and measured (points) cuts of the top ten under chunks and dealing.}
  \Description{Two stacked charts sharing an x axis, the mean retriever rank of the sliding window's top ten, running from 50 on the left to 5 on the right, where retrieval is better, marked better with an arrow. A one-line key above them: solid line, the uniform model of Proposition 1; dashed line, Mallows fit; hollow points BM25, filled points dense; large points, pooled. Top chart, on a blue panel, titled Chunks cut more as retrieval improves, 0 to 6 passages cut: a faint dealing curve lies along the floor, and the chunk curve of Proposition 1 rises from 0.15 to its maximum of 6 as retrieval improves, the dashed Mallows curve rises above it, and eighteen small benchmark points follow the dashed curve; two large points mark the pooled values, 2.0 for BM25 and 2.8 for the dense retriever. Bottom chart, on an orange panel, titled Dealing cuts about 0.1 (y stretched 25 times), 0 to 0.2 passages cut: a dotted random-split line at 0.149, the dealing curve of Proposition 1 falling from 0.149 to 0 with the dashed Mallows curve beside it, eighteen small benchmark points scattered around it, one above the random line, and two large points for the pooled values on dealt input, 0.09 for BM25 and 0.06 for the dense retriever.}
  \label{fig:prior}
\end{figure}


==> figures/fig3.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig3_forest.pdf}
  \caption{nDCG@10 with dealt minus contiguous groups (random for JointRank), with paired 95\% CIs.}
  \Description{A forest plot in two panels, BM25 and the dense retriever Qwen3-Embedding-4B, sharing one horizontal axis of nDCG@10 difference from minus 4 to plus 6 points. Marks are orange where dealing gains significantly, grey where the interval crosses zero, and dark where dealing loses. Rows are schedules grouped into two blocks. Where a quota can bind, on a shaded band: DealRank's round 1 gains 2.7 points over BM25 and 4.4 over the dense retriever, TourRank at every stage 2.2 and 4.5, and BlitzRank at w=20 on dealt input changes by about minus 0.2 and minus 0.4 points, not significant, while making 0.46 and 0.57 fewer calls on 100-candidate queries, written in orange under its row. Where no quota can bind: TourRank's first stage, BlitzRank at w=10, ListK and TDPart sit within 0.6 points of zero with intervals that cross it, and BlitzRank at w=10 makes 0.45 and 0.59 more calls. JointRank's block design changes by minus 0.8 points over BM25, not significant, and by minus 2.1 points over the dense retriever, an interval from minus 4.85 to minus 0.01.}
  \label{fig:schedules}
\end{figure}


==> sections/method.tex <==
\section{Quotas and Splits}
\label{sec:method}

\paragraph{Setting.} A retriever returns $N$ candidates with its own ordering. It passes these candidates to an LLM functioning as a listwise ranker which takes windows containing a query and at most $w$ passages (for comparability, we use $w{=}20$, as in prior work~\cite{sun2023rankgpt,blitzrank2026}) and returns their permutation. A schedule decides how the individual LLM calls are orchestrated, and issues calls in rounds, each depending only on earlier rounds. Listwise reranking latency is defined as the sum over rounds of the slowest call in each.

\paragraph{Groups and quotas.} In a parallel round, candidates are split into $H$ groups of at most $w$ documents, and each group is ranked in one individual call, advancing a \emph{\textbf{quota}} of its top $q$. Suppose the ranker is \emph{consistent}, ordering every call by one fixed ranking whose top~$k$ we call the true top~$k$. A true top-$k$ passage is then cut only when its group holds more than $q$ of them. Thus, if $T$ is the set of their retriever ranks, a split into groups $P_1,\ldots,P_H$ cuts $\sum_h(|T\cap P_h|-q)_+$, where $(x)_+=\max(x,0)$. The quota \emph{can bind} when $q<k$, and only then does the split decide what is cut. In practice, whether or not quotas can bind depends on the schedule used: for the top ten, they can bind in BlitzRank's merge call at $w{=}20$ as well as in DealRank, which both take four passages from each group of twenty, and in TourRank's second stage, which advances four of ten, but not in TourRank's first stage, which advances ten of twenty. TDPart~\cite{parry2024tdpart} and ListK's quickselect~\cite{listk2026} have no quota, since a passage advances whenever it beats a pivot, and neither does BlitzRank in its $w{=}10$ setting, which merges its blocks one passage per block at a time.

\paragraph{Splits.} \emph{Contiguous chunks} give group~$i$ the retriever's ranks $(i{-}1)w{+}1$ to $iw$, as in BlitzRank's default implementation. A \emph{random partition} assigns ranks to groups uniformly at random, and \textbf{\emph{dealing}} gives group~$i$, which we then call a hand, the ranks $i, i{+}H, i{+}2H, \ldots$

\input{tables/main_gemini}
\input{figures/fig2}

\paragraph{Expected cuts.}
\label{sec:why}
A dealt hand holds exactly $q$ of the retriever's top $Hq$ ranks, meaning that, on every list, dealing cuts at most as many of the true top~$k$ as the retriever ranked below $Hq$, and none when $T$ lies within the top $Hq$. Proposition~\ref{prop:deal} compares the three splits on average, in a simple model where retriever quality is a single depth~$R$. The true top~$k$ is a uniformly random set of $k$ ranks within the retriever's top~$R$, so a smaller $R$ means a better retriever.

\begin{proposition}
\label{prop:deal}
Let $T$, the retriever ranks of a consistent ranker's top~$k$ ($q<k\le w$), be uniform over the $k$-subsets of the retriever's top~$R$, and let $\ell_P(R)$ be the expected number cut by a split~$P$ of the candidates into at most $H$ groups, of any sizes, that each advance their top~$q$. For every~$R$, dealing minimizes $\ell_P(R)$ over all splits, and $\ell_{\mathrm{deal}}(R)\le\ell_{\mathrm{rand}}\le\ell_{\mathrm{chunk}}(R)$, where $\ell_{\mathrm{rand}}=H\,\mathbb{E}(X-q)_+$, $X\sim\mathrm{Hyp}(Hw,k,w)$ counts the true top~$k$ in a random group, is the loss of a uniformly random partition into $H$ groups of~$w$, drawn independently of~$T$, under any law of~$T$. As $R$ shrinks, $\ell_{\mathrm{deal}}$ falls to $0$ for $R\le Hq$ and $\ell_{\mathrm{chunk}}$ rises to $k-q$ for $R\le w$.
\end{proposition}

\noindent\emph{Sketch.} The expected loss is $\sum_h g(c_h)$, where $c_h$ is the number of group $h$'s ranks within the top~$R$ and $g(c)=\mathbb{E}(X-q)_+$ for $X\sim\mathrm{Hyp}(R,k,c)$. Since $g$ is convex, the balanced counts that dealing has at every~$R$ are optimal, and the only splits balanced at every~$R$ deal each run of $H$ consecutive ranks one to each group, in some order, as in a snake draft. Coupling depths $R$ and $R{+}1$ shows the loss rises when rank $R{+}1$ joins a least-filled group of an evenly split prefix, as in dealing, and falls when every other group is full or empty, as in chunking. Groups of~$w$ agree at $R{=}N$.\qed


\noindent Chunks thus cut more passages as the retriever improves, and dealt hands cut fewer. With five groups of twenty and $k{=}10$, chunks lose $6$ passages at $R=20$, $2.9$ at $R=30$ and $1.1$ at $R=50$, against $0$, $0.05$ and $0.10$ for dealing. A random partition loses $0.149$ in expectation on every list, as in approximate top-$k$~\cite{samaga2025approxtopk}, which with a consistent ranker is the most that dealing can gain over it at this quota, and we therefore expect the two to differ little there. A random partition's loss does not shrink as the retriever improves, so under a perfect retriever it still cuts a top-ten passage in 12.7\% of queries. It loses $0.69$ when ten groups of ten keep two and $1.68$ when twenty groups of five keep one.

The result covers any retriever under which each set $T$ has a probability that depends only on its deepest rank and does not increase with it, and a noisy ranker whose call advances on average $a(x)$ of the $x$ top-$k$ passages it holds, whenever $a$ is concave. Measured against the sliding window's top ten in 51{,}955 Gemini calls, $a$ is concave up to $x{=}7$, and under the measured curve dealing remains optimal at every depth from 10 to 100. Figure~\ref{fig:prior} compares these losses with measured cuts. Importantly, Proposition~\ref{prop:deal} bounds cuts of the ranker's own top ten, not nDCG@10, which is measured separately in \S\ref{sec:results}.

\subsection{DealRank}
\label{sec:dealrank}

Only a call that holds both of the two best passages can order them, which bounds the calls that any schedule needs, thus:

\begin{proposition}
\label{prop:rounds}
Let the ranker be consistent, $N{=}Hw$ with $H\ge2$, and $Hq\le w$. Over any split into $H$ groups of~$w$, two rounds return the true top~$q$ exactly on every list in $H{+}1$ calls, the fewest with which any schedule returns even the best passage on every list, since a call eliminates at most $w{-}1$ passages, as in pairwise selection~\cite{valiant1975,braverman2016parallel}. One round does so only if every two candidates share a call, which takes at least $H(H{+}1)$ calls~\cite{schonheim1964coverings}.
\end{proposition}

\noindent This guarantee covers the top~$q$, which is four of the ten passages that nDCG@10 scores in our setting. The other six carry no worst-case guarantee, and their expected cuts are those of Proposition~\ref{prop:deal}. We subsequently introduce \textbf{DealRank}, a simple scheduling method built on these findings. It implements the proposed, low-round-count schedule of Proposition~\ref{prop:rounds} on a dealt split, with no repair round. In our $w{=}20$ evaluation setting, it is a two-round schedule: for $N{=}100$, it deals the candidates into $H{=}5$ hands of twenty, each presented in retriever order, ranks the hands concurrently and advances the top $q{=}4$ of each to the final ranking call, which lists them by their place in their hand, then by retriever rank. At higher $N$ values, it follows the same logic but becomes \emph{hierarchical}, re-ordering $N{=}1000$ documents in just 3 rounds by first creating $H{=}50$ hands that each keep $q{=}2$, which are then re-dealt, still in retriever order, into $H{=}5$ hands, whose $q{=}4$ candidates advance to the final ranking call in retriever order. For $N{=}500$, 25 hands keep 3, then 4 hands keep 5. Candidates eliminated in later rounds are ranked above those eliminated earlier, and within a round by their place in their hand, then by retriever rank.


==> sections/results.tex <==
\section{Experimental Setup}
\label{sec:setup}


\paragraph{Data and Metrics.} We use standard evaluation suites: TREC-DL19~\cite{craswell2020trecdl} and DL20~\cite{craswell2021trecdl} built upon the MS MARCO passage collection~\cite{nguyen2016msmarco}, as well as 8 widely used sets from the BEIR~\cite{thakur2021beir} collection\footnote{Selected to follow previous studies on listwise scheduling, facilitating validation of our results against previously reported ones.}, totaling 1{,}622 queries. The first stage is the BM25 top 100 from the Pyserini~\cite{lin2021pyserini} runs released with RankLLM~\cite{sharifymoghaddam2025rankllm}. For the experiments targeting first stage quality comparisons, we use dense embedding Qwen3-Embedding-4B~\cite{zhang2025qwen3embedding} on all benchmarks but Signal and News.\footnote{Their corpora are not publicly available, and no pre-built pools exist for them.} We report macro-averaged nDCG@10 with paired 95\% bootstrap intervals resampling benchmarks, then queries.

\paragraph{Models and Schedules.} All methods share the RankGPT prompt~\cite{sun2023rankgpt} and LLMs are called at temperature 0 with reasoning disabled. We use Gemini~3~Flash\footnote{Following \citet{blitzrank2026}} for the main evaluation results, and six more, spanning open and closed models, to assess generalization. On Gemini, we average three runs of DealRank, the sliding window and BlitzRank $w{=}20$, and ten seeds of the random partition. As for schedules, baseline schedules are the sliding window (window 20, stride 10)~\cite{sun2023rankgpt}; TourRank with one tournament~\cite{chen2025tourrank}, the variant closest to DealRank's call budget, adapted to the shared permutation prompt;\footnote{As in BlitzRank's evaluation~\cite{blitzrank2026}, we run a single tournament. There, a second tournament doubles TourRank's tokens for 0.6 nDCG@10 points and still trails one sliding-window pass. TourRank's default of ten would take roughly 130 calls and 481k tokens per query in our setting, against DealRank's 6.0 and 31k.} TDPart~\cite{parry2024tdpart}; JointRank~\cite{dedov2025jointrank}; ListK's quickselect~\cite{listk2026}; and BlitzRank~\cite{blitzrank2026}, whose passages per call, its $k$, we write as $w$.\footnote{With the authors' released package and our sliding window, we reproduce BlitzRank's reported results within 0.3 points at $w{=}20$. Other LLMs use our code.}

\paragraph{Timing.} For controlled timing, we serve Qwen3.8-27B in bfloat16 with vLLM~0.33 on two H100s without prefix caching, and run every method on the 43 DL19 queries one at a time, over three repeats. For latency and throughput, we also run DL19, DL20, TREC-COVID and Touch\'{e} with 1, 8 or 32 queries in flight on three server instances, and the DL19 top 500 and 1{,}000 one query at a time (sequential schedules once). Additionally, API latency is timed 3 times, as described in \S\ref{sec:method}.

\input{tables/models}

\section{Results}
\label{sec:results}

We present the results of various schedules applied to Gemini 3 Flash, averaged over 3 runs, in Table~\ref{tab:main-gemini}.

We first observe that every multi-round schedule, other than DealRank on chunks, is within 0.9 points of DealRank, and only TourRank differs from it significantly, despite DealRank's naive framing. Instead, schedules differ in cost: they take up to 13.4 rounds and 48k tokens per query, where DealRank takes 2.0 and 31k. We observe that this trend holds across LLMs, as presented in Table~\ref{tab:models}, where neither BlitzRank nor the sliding window is ahead by more than 0.09 [$-$0.43, $+$0.67] points on average and no per-LLM comparison finds DealRank significantly worse, suggesting DealRank's single final call suffices on average. The intervals support non-inferiority on average over LLMs, though not for every LLM taken alone. At nDCG@20, DealRank is level with the sliding window on Gemini~3~Flash ($-$0.1 [$-$1.5, $+$1.2]). JointRank's single round is 1.8 [0.3, 3.9] points behind DealRank, in line with Proposition~\ref{prop:rounds} on the importance of rounds.


\paragraph{Dealing inside other schedules.} We next focus on whether the use of dealing inside existing schedules improves performance. We measure this on five other schedules with Gemini~3~Flash, and present our results in  Figure~\ref{fig:schedules}. We find that dealing helps wherever a quota can bind. TourRank already deals, but takes 13.0 calls in 5.0 rounds and is 1.44 [0.49, 2.72] points behind DealRank across the three LLMs it ran on (Gemini~3~Flash, DeepSeek V4-Flash and Qwen3.5-35B-A3B). Contiguous groups would cost it a further 2.2 [1.0, 3.6] points over BM25 and 4.5 [2.4, 7.0] over the dense retriever, since its second stage advances four of every ten. BlitzRank at $w{=}20$ instead saves 0.46 to 0.57 calls per query: in its default setting, it triggers its certification call on 59\% of 100-candidate queries, against just 14\% on dealt inputs, with no significant change in nDCG@10 ($-$0.2 [$-$1.0, $+$0.8]). Given dealt input, it is thus essentially DealRank followed by an occasional certification round. Where no quota can bind, in TDPart, ListK, BlitzRank at $w{=}10$ and TourRank's first stage, dealing changes nDCG@10 by at most 0.6 points and never significantly. Dealing lowers nDCG@10 in one schedule only, JointRank, in line with our expectation that dealing's effectiveness is tied to quotas and multi-round processes, as group composition can matter without any quota~\cite{grouprank2025}.


\paragraph{Dealing against other splits.}
\label{sec:mechanism}
As Proposition~\ref{prop:deal} predicts, contiguous chunks result in a significant performance loss of 2.7 nDCG@10 points, and this gap widens with a better retriever. In Figure~\ref{fig:schedules}, we show that on the dense retriever pool (all evaluation, minus Signal and News), chunks cost 4.4 points over the dense retriever and 2.3 over BM25, a difference of 2.1 [0.2, 4.1]. Measured cuts follow the same pattern, as chunks put 2.0 of the sliding window's top ten over their group's quota over BM25 and 2.8 over the dense retriever, where dealt hands put about 0.1, as shown in Figure~\ref{fig:prior}.

A random partition, on the other hand, appears equivalent to dealing at a quota of four, where it differs from DealRank by $-$0.3 [$-$0.8, $+$0.2] points over ten seeds. This is expected, as dealing can gain at most 0.149 passages per query over it there (\S\ref{sec:method}). Per query, its groups hold only 0.07 more of the sliding window's top ten beyond their quota than dealt hands do, and it brings 0.07 [$-$0.01, $+$0.15] fewer of them to the final call, which is too few to show in aggregated nDCG@10. The bound of 0.149 rises to 0.69 and 1.68 passages at quotas of two and one, and the measured deficit grows with it. With Qwen3.8-27B over the dense retriever, it goes from a non-significant 0.0 and 0.3 points at quotas of four and two to 1.3 [0.4, 2.4] at a quota of one, and over BM25 it is smaller and not significant. Even at a quota of four, a random partition is balanced only on average. A dealt hand holds exactly four of the BM25 top twenty, and so at most four of its judged-relevant passages, whereas a random partition places 12\% of these relevant passages in a group holding five or more of them. Such passages reach the final call 8.0 [4.8, 11.0] percentage points less often than when dealt if their group holds five, and 16.5 [11.0, 23.1] less often if it holds six or more. Its results also depend on the seed, where a dealt split is fixed, and the standard deviation of a query's nDCG@10 across three seeds, averaged over every three of the ten, exceeds that of three repeated DealRank runs by 0.72 [0.43, 1.05] points.

\input{figures/fig3}
\input{tables/depth}

\paragraph{Rounds and latency.} BlitzRank in its original form~\cite{blitzrank2026} issues its calls one at a time, which is inefficient. We instead also time it with its first calls run concurrently, a variant we call concurrent BlitzRank. Over the Gemini API, we observe that DealRank's median latency is 3.4 seconds, against 4.0 for concurrent BlitzRank and 13.4 for the sliding window (Figure~\ref{fig:hero}), measured on live concurrent calls and within 0.3 seconds of wall-clock. On dealt input, concurrent BlitzRank takes 3.5 seconds, confirming that the split, and the resulting required certifications, accounts for most of its gap to DealRank. On local timings, with one query in flight on four benchmarks, concurrent BlitzRank takes on average 1.20 [1.14, 1.26] times as long per query as DealRank, or 1.03 [1.01, 1.05] times on dealt input, and the sliding window 3.31 [2.96, 3.69] times. Importantly, DealRank's number of rounds is also predictable: it always takes two, and its 90th percentile is at most 0.36 seconds above its median on every benchmark, while that of concurrent BlitzRank is up to 1.23 seconds above. With 8 or 32 queries in flight, where rounds no longer set the wait alone, DealRank still serves 1.09 [1.06, 1.13] and 1.15 [1.10, 1.20] times the queries per second of concurrent BlitzRank. It serves 1.92 [1.86, 1.97] and 1.54 [1.51, 1.58] times those of the sliding window, and 1.01 [0.99, 1.02] and 1.05 [1.01, 1.10] times those of BlitzRank on dealt input, so most of the gain comes from the split.

\paragraph{Scaling to 1{,}000 candidates.} The gap in rounds widens considerably as the list grows (Table~\ref{tab:depth}). In its hierarchical form, DealRank takes three rounds for 500 and for 1{,}000 candidates alike. At 1{,}000 candidates, concurrent BlitzRank averages 5.7 rounds, and the sliding window 99. These extra rounds buy no measurable quality, with all three schedules staying within 0.4 nDCG@10 points of one another with no significant difference at any list size. A DL19 query over 1{,}000 candidates takes DealRank 10.3 seconds, concurrent BlitzRank 1.26 [1.25, 1.28] times as long, and the sliding window 11.2 [11.1, 11.4] times. Concurrent BlitzRank's gap in time is smaller than its gap in rounds because both schedules spend most of their time in a first round of 50 calls. As candidate size grows, DealRank remains faster and more round-efficient than other methods.

\section{Conclusion}

In this short paper, we analyzed the importance of listwise scheduling across both quality and efficiency metrics. We demonstrated that many existing schedules reach similar ranking performance, but with widely varying levels of both token and time requirements. Building upon this, we formulated the importance of per-round quotas and demonstrated that the split of parallel listwise schedules greatly matters where a group's quota can bind. We showed that dealing is optimal in expected cuts under a simple retriever model and, unlike a random partition, is balanced on every query. DealRank, a naive schedule built upon these observations, is a robust schedule which appears competitive with all strong existing methods with higher efficiency and higher predictability. DealRank is also highly scalable, retaining round predictability and lower latencies even with 500 and 1{,}000 candidates. Its latency gain over concurrent BlitzRank is modest but consistent, between 1.1 and 1.4 times at every list size, and reaches eleven times over the sliding window at 1{,}000 candidates. Our intervals rule out average deficits above 0.7 nDCG@10 points, though not differences of about a point on a single LLM. Additionally, applying dealt splits to existing state-of-the-art methods such as BlitzRank improves their efficiency by reducing the frequency of repair rounds, thus improving average latency.

==> tables/depth.tex <==
% Generated by paper/analysis/depth_table.py (sources in its docstring); numbers in analysis/out/depth_table.json.
\begin{table}[t]
\caption{Deeper lists on DL19, DL20, DBpedia and SciFact with Qwen3.8-27B. $\parallel$: concurrent first calls.}
\label{tab:depth}
\centering\small
\setlength{\tabcolsep}{3.1pt}
\begin{tabular}{@{}r rrr rrrr@{}}
\toprule
 & \multicolumn{3}{c}{nDCG@10} & \multicolumn{4}{c}{Seconds per DL19 query (rounds)} \\
\cmidrule(lr){2-4}\cmidrule(l){5-8}
Top & \textbf{Deal} & Blitz & Window & \textbf{Deal} & Blitz\,$\parallel$ & Blitz & Window \\
\midrule
100 & 67.9 & 67.6 & 67.5 & \textbf{2.9}$_{2}$ & 4.0$_{2.6}$ & 8.2$_{6.6}$ & 10.6$_{9}$ \\
500 & 69.8 & 69.9 & 70.1 & \textbf{7.0}$_{3}$ & 8.0$_{4.3}$ & 33.0$_{28}$ & 57.9$_{49}$ \\
1{,}000 & 71.0 & 70.8 & 70.8 & \textbf{10.3}$_{3}$ & 13.0$_{5.7}$ & 65.1$_{55}$ & 115.4$_{99}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/main_gemini.tex <==
% auto-generated by paper/analysis/tables.py -- do not edit
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{0.94}
\caption{Schedules on Gemini~3~Flash over the BM25 top 100 (nDCG@10$\times$100). p50, p90: local Qwen3.8-27B latency in seconds (\S\ref{sec:setup}). $^\dagger$First calls run concurrently. Bold: best reranker, among multi-call methods for costs.}
\label{tab:main-gemini}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l>{\columncolor{avgcol}}r>{\columncolor{avgcol}}l@{\hspace{8pt}}rrrrrrrrrr@{\hspace{8pt}}rrrrrr@{}}
\toprule
& \multicolumn{2}{c}{\cellcolor{avgcol}} & \multicolumn{10}{c}{nDCG@10 $\times$ 100 per benchmark} & \multicolumn{6}{c}{Cost per 100-candidate query} \\
\cmidrule(lr){4-13}\cmidrule(l){14-19}
Method & \textbf{Avg.} & $\Delta$ vs.\ DealRank & DL19 & DL20 & COVID & NFC & Signal & News & Rob04 & Touch\'{e} & DBP & SciF & Calls & Rounds & Max & Tok.\ (k) & p50 & p90 \\
\midrule
BM25 & 44.7 & $-$12.9 {\scriptsize[$-$19.7, $-$5.6]} & 50.6 & 48.0 & 59.5 & 32.2 & 33.1 & 39.5 & 40.7 & 44.2 & 31.8 & 67.9 & 0 & 0 & 0 & 0 & \hfil--\hfil & \hfil--\hfil \\
Top-20 only (one call) & 53.8 & $-$3.8 {\scriptsize[$-$7.2, $-$0.1]} & 66.1 & 64.2 & 75.2 & 37.2 & \textbf{35.5} & 45.3 & 54.2 & \textbf{42.6} & 40.0 & 77.9 & 1.0 & 1.0 & 1 & 5.2 & 1.18 & 1.21 \\
Sliding window & \textbf{57.9} & +0.3 {\scriptsize[$-$0.4, +0.9]} & 74.6 & \textbf{73.0} & 82.6 & \textbf{39.5} & 33.7 & 49.0 & \textbf{65.2} & 35.0 & \textbf{46.1} & \textbf{80.6} & 9.0 & 9.0 & 9 & 46.1 & 10.63 & 10.78 \\
TourRank $r{=}1$ & 56.7 & $-$0.9 {\scriptsize[$-$1.9, $-$0.1]} & 73.5 & 71.2 & 81.7 & 38.7 & 33.4 & 48.5 & 64.3 & 32.5 & 45.1 & 77.9 & 13.0 & 5.0 & 5 & 48.1 & 4.53 & 4.63 \\
TDPart & 57.1 & $-$0.5 {\scriptsize[$-$1.8, +0.9]} & 72.9 & 70.0 & 82.1 & 38.7 & 34.7 & 48.8 & 62.1 & 37.8 & 44.7 & 79.1 & 6.9 & 2.9 & 3 & 31.6 & 3.89 & 4.05 \\
JointRank $r{=}4$ (one round) & 56.0 & $-$1.6 {\scriptsize[$-$3.7, $-$0.0]} & 73.2 & 72.3 & 82.3 & 38.4 & 32.7 & \textbf{50.1} & 63.8 & 31.8 & 43.7 & 71.5 & 20.0 & \textbf{1.0} & \textbf{1} & 102.8 & 3.60 & 3.89 \\
BlitzRank $w{=}10$ & 57.3 & $-$0.3 {\scriptsize[$-$1.2, +0.3]} & 74.6 & 71.6 & 82.8 & 39.1 & 33.1 & 48.2 & 64.7 & 33.3 & 45.4 & 79.9 & 13.4 & 13.4 & 15 & 35.2 & 7.12 & 7.69 \\
BlitzRank $w{=}20$ & 57.8 & +0.2 {\scriptsize[$-$0.5, +1.0]} & \textbf{75.1} & 71.8 & \textbf{83.1} & 38.8 & 33.7 & 48.5 & 64.6 & 36.2 & \textbf{46.1} & 80.1 & 6.6 & 6.6 & 7 & 33.8 & 8.24 & 8.39 \\
BlitzRank $w{=}20$, concurrent$^\dagger$ & 57.8 & +0.2 {\scriptsize[$-$0.5, +1.0]} & \textbf{75.1} & 71.8 & \textbf{83.1} & 38.8 & 33.7 & 48.5 & 64.6 & 36.2 & \textbf{46.1} & 80.1 & 6.6 & 2.6 & 3 & 33.8 & 4.00 & 4.16 \\
\midrule
DealRank on contiguous chunks & 54.9 & $-$2.7 {\scriptsize[$-$4.0, $-$1.6]} & 70.2 & 69.1 & 81.9 & 37.2 & 28.7 & 45.9 & 62.3 & 30.7 & 44.1 & 78.9 & \textbf{6.0} & 2.0 & 2 & \textbf{30.8} & \textbf{2.88} & \textbf{2.96} \\
\midrule
\rowcolor{dealrow}BlitzRank $w{=}20$, dealt, concurrent$^\dagger$ & 57.6 & $-$0.0 {\scriptsize[$-$0.8, +1.0]} & 74.1 & 72.3 & 82.9 & 38.6 & 33.0 & 48.0 & 63.8 & 37.9 & 45.6 & 79.8 & 6.1 & 2.1 & 3 & 31.5 & 2.89 & 3.14 \\
\rowcolor{dealrow}DealRank, random partition & 57.4 & $-$0.3 {\scriptsize[$-$0.8, +0.2]} & 74.0 & 71.8 & 82.4 & 39.1 & 32.5 & 49.0 & 64.4 & 34.2 & 45.8 & 80.4 & \textbf{6.0} & 2.0 & 2 & 30.9 & \textbf{2.88} & \textbf{2.96} \\
\rowcolor{dealrow}\textbf{DealRank} & 57.6 & \hfil--\hfil & 74.4 & 72.1 & \textbf{83.1} & 39.0 & 32.8 & 49.1 & 64.7 & 35.2 & 45.5 & 80.3 & \textbf{6.0} & 2.0 & 2 & 30.9 & \textbf{2.88} & \textbf{2.96} \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/models.tex <==
% auto-generated by paper/analysis/tables.py -- do not edit
\begin{table}[!b]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\caption{DealRank's nDCG@10$\times$100 on six LLMs, and each schedule's difference to it (95\% CI on the average). $^\dagger$Frontier-model check against BlitzRank $w{=}10$ only (---: not run), left out of the average.}
\label{tab:models}
\resizebox{\ifdim\width>\columnwidth\columnwidth\else\width\fi}{!}{%
\begin{tabular}{@{}lrccccc@{}}
\toprule
& & \multicolumn{2}{c}{BlitzRank} & Sliding & & JointRank \\
Model & DealRank & $w{=}20$ & $w{=}10$ & window & TDPart & $r{=}4$ \\
\midrule
DeepSeek V4-Flash & 58.5 & $-$1.01 & $-$0.50 & $-$0.10 & $-$0.36 & $-$3.12 \\
Qwen3.5-35B-A3B & 56.7 & $-$0.22 & $-$0.42 & $-$0.62 & $-$0.35 & $-$1.87 \\
Qwen3.8-27B & 56.9 & +0.61 & +0.79 & $-$0.26 & $-$0.15 & $-$1.05 \\
Kimi K2.6 & 57.3 & +0.75 & +0.57 & +0.52 & $-$0.14 & $-$1.18 \\
GLM-5.2 & 57.2 & +0.20 & +0.37 & +0.74 & $-$0.17 & $-$1.85 \\
Gemini 3 Flash & 57.6 & +0.20 & $-$0.35 & +0.30 & $-$0.50 & $-$1.61 \\
GPT-5.5$^\dagger$ & 57.8 & --- & +0.33 & --- & --- & --- \\
\midrule
Average (excl.\ GPT-5.5) & 57.4 & +0.09 & +0.08 & +0.09 & $-$0.28 & $-$1.78 \\
 & & {\footnotesize[$-$0.43,+0.67]} & {\footnotesize[$-$0.43,+0.59]} & {\footnotesize[$-$0.5,+0.6]} & {\footnotesize[$-$1.2,+0.7]} & {\footnotesize[$-$3.9,$-$0.3]} \\
\bottomrule
\end{tabular}}
\end{table}

